Certifiably Globally Optimal Extrinsic Calibration from Per-Sensor Egomotion

We present a certifiably globally optimal algorithm for determining the extrinsic calibration between two sensors that are capable of producing independent egomotion estimates. This problem has been previously solved using a variety of techniques, including local optimization approaches that have no formal global optimality guarantees. We use a quadratic objective function to formulate calibration as a quadratically constrained quadratic program (QCQP). By leveraging recent advances in the optimization of QCQPs, we are able to use existing semidefinite program (SDP) solvers to obtain a certifiably global optimum via the Lagrangian dual problem. Our problem formulation can be globally optimized by existing general-purpose solvers in less than a second, regardless of the number of measurements available and the noise level. This enables a variety of robotic platforms to rapidly and robustly compute and certify a globally optimal set of calibration parameters without a prior estimate or operator intervention. We compare the performance of our approach with a local solver on extensive simulations and multiple real datasets. Finally, we present necessary observability conditions that connect our approach to recent theoretical results and analytically support the empirical performance of our system.

==> macros.tex <==
% Matt's additions
% Norms
\newcommand{\norm}[2]{\|#1\|_{#2}}
\newcommand{\frob}[1]{\|#1\|_{\scriptscriptstyle F}}

% Bold for matrix/vector variables
\newcommand{\mbf}[1]{\mathbf{#1}}
%\newcommand{\ones}[1]{\mathbf{1}_{#1}}
%\newcommand{\vect}[1]{\text{vec}(#1)}

\newcommand{\GG}{\mathcal{G}}
\newcommand{\GGi}{\mathcal{G}_{\normalfont\text{init}}}
\newcommand{\LLi}{\mathbf{L}_{\normalfont\text{init}}}
\newcommand{\Hgraph}{\mathcal{H}}
\newcommand{\GGQ}{\mathcal{G}_{[\mathcal{Q}]}}
\newcommand{\OPT}{\mathsf{OPT}}
\newcommand{\opt}{\mathsf{opt}}
\newcommand{\GRD}{{\normalfont\text{greedy}}}
\newcommand{\Gbb}{\mathbb{G}}
\newcommand{\esp}{$\mathrm{ESP}$}
\newcommand{\desp}{${\mathrm{ESP}^\ast}$}
\newcommand{\GGc}{{G}^\circ}
\newcommand{\EEc}{{E}^\circ}
\newcommand{\EEi}{{\EE}_{\normalfont\text{init}}}
\newcommand{\rvp}{\mathbf{r_\mathrm{vp}}}
\newcommand{\Jvp}{\mathbf{J_\mathrm{vp}}}
\newcommand{\JvpK}{\mathbf{J_\mathrm{vp}^\mathrm{K}}}
\newcommand{\VV}{\mathcal{V}}
\newcommand{\TT}{\mathcal{T}}
\newcommand{\T}{{T}}
\newcommand{\K}{{K}}
%\newcommand{\EE}{{\large\mathpzc{E}}}
\newcommand{\EE}{{\mathcal{E}}}
\newcommand{\xx}{\mathbf{x}}
\newcommand{\sss}{\mathbf{s}}
\newcommand{\cc}{\mathbf{c}}
\newcommand{\qq}{\mathbf{q}}
\newcommand{\dd}{\mathbf{d}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\uu}{\mathbf{u}}
\newcommand{\zero}{\mathbf{0}}
\newcommand{\ones}{\mathbf{1}}
\newcommand{\ff}{{f}}
\newcommand{\LL}{\mathbf{L}}
\newcommand{\LLo}{\mathbf{L}_\circ}
\newcommand{\KK}{\mathbf{C}}
\newcommand{\KKK}{\mathcal{K}}
\newcommand{\DD}{\mathbf{D}}
\newcommand{\MM}{\mathbf{M}}
\newcommand{\NN}{\mathbf{N}}
\newcommand{\PP}{\mathbf{P}}
\newcommand{\ES}{\mathbf{S}}
\newcommand{\HH}{\mathbf{H}}
\newcommand{\cHH}{\mathcal{H}}
\newcommand{\cSS}{\mathcal{S}}
\newcommand{\bHH}{\tilde{\mathbf{H}}}
\newcommand{\bKs}{\bHH_1^\dagger}
\newcommand{\bJJ}{\tilde{\mathbf{J}}}
\newcommand{\WW}{\mathbf{W}}
\newcommand{\rr}{\mathbf{r}}
\newcommand{\yy}{\mathbf{y}}
\newcommand{\brr}{\tilde{\mathbf{r}}}
\newcommand{\zz}{\mathbf{z}}
\newcommand{\bzz}{\tilde{\mathbf{z}}}
\newcommand{\ww}{\boldsymbol\epsilon}
\newcommand{\hh}{\mathbf{h}}
\newcommand{\pp}{\mathbf{p}}
\newcommand{\ppp}{\boldsymbol\pi}
\newcommand{\AAA}{\mathbf{A}}
\newcommand{\AAAtop}{\AAA^{\hspace{-0.1cm}\top}}
\newcommand{\AAo}{\mathbf{A}_\circ}
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Aintra}{\mathcal{A}_\text{\normalfont intra}}
\newcommand{\Ainit}{\mathcal{A}_\text{\normalfont init}}
\newcommand{\Ainter}{\mathcal{A}_\text{\normalfont inter}}
\newcommand{\Mintra}{\mathcal{M}_\text{\normalfont intra}}
\newcommand{\Minter}{\mathcal{M}_\text{\normalfont inter}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\aaa}{\mathbf{a}}
\newcommand{\ee}{\mathbf{e}}
\newcommand{\BB}{\mathbf{A}_\text{odo}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\II}{\mathbf{I}}
\newcommand{\RR}{\mathbf{R}}
\newcommand{\CC}{\boldsymbol\Sigma}
\newcommand{\CCC}{\mathcal{C}}
\newcommand{\QQ}{\mathbf{Q}}
\newcommand{\cRR}{\mathbf{\Gamma}}
\newcommand{\cQQ}{\mathcal{Q}}
\newcommand{\tSS}{\mathbf{S}}
\newcommand{\tRR}{\tilde{\mathbf{R}}}
\newcommand{\OO}{{\Omega}}
\newcommand{\DDD}{\boldsymbol{\Delta}}
\newcommand{\trr}{\mathbf{\tilde{\rr}}}
\newcommand{\thth}{{\boldsymbol\theta}}
\newcommand{\mumu}{{\boldsymbol\mu}}
\newcommand{\bRR}{\mathbf{\bar{{R}}}}
\newcommand{\tJJ}{\mathbf{\tilde{J}}}
\newcommand{\JJ}{\mathbf{{J}}}
\newcommand{\Zcal}{{\mathcal{Z}}}
\newcommand{\III}{\mathkk{I}}
\newcommand{\bII}{\bar{\mathbf{\mathcal{I}}}}
%\newcommand{\logtree}{\mathsf{LogTree}_{n,w}}
\newcommand{\logtree}{\tau_{n,w}}
%\newcommand{\tree}{\mathsf{Tree}_{n,w}}
\newcommand{\tree}{t_{n,w}}
\newcommand{\logTG}{\Phi_{w}}
\newcommand{\logtreeu}{\mathsf{Log\,Tree}_{n}}
\newcommand{\treeu}{\mathsf{tree}_{n}}
\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}
\newcommand{\HHH}{\mathbfcal{H}}
\newcommand{\Rset}{\mathbb{R}}
\newcommand{\Exp}{\mathbb{E}}
\newcommand{\Nset}{\mathbb{N}}
\newcommand{\ksucc}{\hspace{-0.1cm}\succ\hspace{-0.1cm}}
\newcommand{\ksucceq}{\hspace{-0.1cm}\succeq\hspace{-0.1cm}}
\newcommand{\ifff}{if and only if}
\newcommand{\RE}{\mathrm{RE}}
\newcommand{\Cov}{\mathbb{C}\mathrm{ov}}
\newcommand{\Inf}{\mathkk{I}}
\newcommand{\np}{n_p}
\newcommand{\nf}{n_f}
\newcommand{\PPP}{\mathbf{\Pi}}
\newcommand{\AAAw}{\mathbf{A}^{\hskip-0.05cm w}}
\newcommand{\AAAwp}{\mathbf{A}^{\hskip-0.05cm w_p}}
\newcommand{\LLw}{\mathbf{L}^{\hskip-0.05cm w}}
\newcommand{\LLwp}{\mathbf{L}^{\hskip-0.05cm w_p}}
\newcommand{\LLwt}{\mathbf{L}^{\hskip-0.05cm w_\theta}}

\newcommand{\gsq}{\textcolor{green}{$\bullet$}}
\newcommand{\ysq}{\textcolor{yellow}{$\bullet$}}
\newcommand{\rsq}{\textcolor{red}{$\bullet$}}
\newcommand{\cg}{\cellcolor{green!10!white}}
\newcommand{\crr}{\cellcolor{red!10!white}}


\DeclareMathOperator{\wrap}{wrap}
\DeclareMathOperator{\card}{card}
\DeclareMathOperator{\vect}{vec}
\DeclareMathOperator{\var}{Var}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\Null}{null}
\DeclareMathOperator*{\range}{range}
\DeclareMathOperator*{\rank}{rank}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\diag}{diag}

\newcommand*{\Scale}[2][4]{\scalebox{#1}{$#2$}}

\newcommand{\Plus}{\texttt{\normalfont +}}
\newcommand{\Minus}{\texttt{-}}
\newcommand{\Cplus}{\CCC^\Plus}
\newcommand{\Cminus}{\CCC^\Minus}
\newcommand{\espPlus}{\mathrm{ESP}^\Plus}
\newcommand{\respPlus}{\mathrm{RESP}^\Plus}
\newcommand{\despPlus}{\mathrm{ESP}^\ast}
\newcommand{\espMinus}{\mathrm{ESP}^\Minus}




\newcommand{\globalmin}{\textsf{\small\bfseries Global Min}}
\newcommand{\localmin}{\textsf{\small\bfseries Local Min}}
\newcommand{\notconverged}{\textsf{\small\bfseries Not Converged}}

\newcommand\Tstrut{\rule{0pt}{2.2ex}}         % = `top' strut
\newcommand\Bstrut{\rule[-0.9ex]{0pt}{0pt}}   % = `bottom' strut


\newcommand{\ggo}{\texttt{g2o}}
\newcommand{\cholmod}{{CHOLMOD}}

\newcommand*{\matminus}{%
  \leavevmode
  \hphantom{0}%
  \llap{%
    \settowidth{\dimen0 }{$0$}%
    \resizebox{1.1\dimen0 }{\height}{$-$}%
  }%
}


\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\kscan}{k_\textsf{register}}
\newcommand{\kfound}{k_\textsf{found}}
\newcommand{\kcomm}{k_\text{\tiny\faWifi}}
\newcommand{\fcomm}{f_\text{\tiny\faWifi}}
\newcommand{\kcomp}{k_\text{\tiny\faLaptop}}
\newcommand{\fcomp}{f_\text{\tiny\faBalanceScale}}
\newcommand{\Gex}{\GG}
\newcommand{\Lcaltotal}{\mathcal{L}_\textsf{total}}
%\let\oldsim\sim
%\renewcommand{\sim}{\overset{\Lcal}{\oldsim}}

\newcommand\kk[1]{\textcolor{blue!80!gray}{\textbf{KK: }\ul{#1}}}
% for Matt
\newcommand\mg[1]{\textcolor{magenta!70!yellow}{\textbf{MG: }\ul{#1}}}


\newcommand{\bipgraph}[2]{%
    \begin{tikzpicture}[every node/.style={circle,fill,scale=0.4,draw}]
    \foreach \xitem in {1,2,...,#1}
    {%
    % first set
    \node at (\xitem,0) (a\xitem) {};
    % second set
    \node at (\xitem,1) (b\xitem) {};   
    }%

    % connections
    \foreach \x [count=\xi] in {#2}
    {% 
    \foreach \tritem in \x % <-- Here no braces to make it a foreach list also not \xi but \x
    \draw(a\xi) -- (b\tritem);
    }
    \end{tikzpicture}  
}

	\newcommand\DoubleLine[5][4pt]{%
	  \path(#2)--(#3)coordinate[at start](h1)coordinate[at end](h2);
	  \draw[<-,line width=0.25mm,black] ($(h1)!#1!90:(h2)$)  to ["#4"]   ($(h2)!#1!-90:(h1)$);
	  \draw[->,line width=0.25mm,black] ($(h1)!#1!-90:(h2)$) to ["#5" '] ($(h2)!#1!90:(h1)$);
	}
	\newcommand\DoubleLineOneDirectional[5][4pt]{%
	  \path(#2)--(#3)coordinate[at start](h1)coordinate[at end](h2);
	  \draw[->,line width=0.75mm,black] ($(h1)!#1!90:(h2)$)  to ["#4"]
	  ($(h2)!#1!-90:(h1)$);
	  \draw[->,very thick,densely dashed,black!50!white, bend right=15] ($(h1)!#1!-100:(h2)$) to
	  ["#5" '] ($(h2)!#1!100:(h1)$);
	}
	\newcommand\xDoubleDashedLine[5][4pt]{%
	  \path(#2)--(#3)coordinate[at start](h1)coordinate[at end](h2);
	  \draw[->,very thick,densely dashed,black!50!white,bend left=90] ($(h1)!#1!90:(h2)$)  to ["#4"]
	  ($(h2)!#1!-90:(h1)$);
	  \draw[<-,very thick,densely dashed,black!50!white, bend right=80] ($(h1)!#1!-100:(h2)$) to
	  ["#5" '] ($(h2)!#1!100:(h1)$);
	}
	\newcommand\DoubleDashedLine[5][4pt]{%
	  \path(#2)--(#3)coordinate[at start](h1)coordinate[at end](h2);
	  \draw[<-,very thick,black!50!white,densely
	  dashed,sloped,anchor=south] ($(h1)!#1!90:(h2)$)  to ["#4"]   ($(h2)!#1!-90:(h1)$);
	  \draw[->,very thick,  black!50!white,densely dashed,sloped,anchor=south] ($(h1)!#1!-90:(h2)$) to ["#5" '] ($(h2)!#1!90:(h1)$);
	}
	\newcommand\DoubleDashedLineRev[5][4pt]{%
	  \path(#2)--(#3)coordinate[at start](h1)coordinate[at end](h2);
	  \draw[<-,very thick,  black!50!white,densely dashed,sloped,anchor=south] ($(h1)!#1!-90:(h2)$) to ["#5" '] ($(h2)!#1!90:(h1)$);
	  \draw[->,very thick,black!50!white,densely dashed,sloped,anchor=south] ($(h1)!#1!90:(h2)$)  to ["#4"]   ($(h2)!#1!-90:(h1)$);
	}



\definecolor{kkGreen}{RGB}{201,232,206}
\definecolor{kkRed}{RGB}{255,196,215}
\definecolor{kkBlue}{RGB}{214,226,255}

